Self-assembling interactive modules: A research programme

In this paper we propose a research programme for getting structural characterisations for 2-dimensional languages generated by self-assembling tiles. This is part of a larger programme on getting a formal foundation of parallel, interactive, distributed systems.

==> chapters/chapterGS/fig/generic-tile.latex <==
\setlength{\unitlength}{4144sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(2338,2338)(857,-2355)
\thicklines
{\color[rgb]{0,0,0}\put(901,-2311){\framebox(2250,2250){}}
}%
{\color[rgb]{0,0,0}\put(1351,-1861){\framebox(1350,1350){}}
}%
{\color[rgb]{0,0,0}\put(901,-61){\line( 1,-1){450}}
}%
{\color[rgb]{0,0,0}\put(3151,-61){\line(-1,-1){450}}
}%
{\color[rgb]{0,0,0}\put(2701,-1861){\line( 1,-1){450}}
}%
{\color[rgb]{0,0,0}\put(1351,-1861){\line(-1,-1){450}}
}%
\put(1801,-1411){\makebox(0,0)[lb]{\smash{{\SetFigFont{34}{40.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}a}%
}}}}
\put(1126,-1636){\makebox(0,0)[lb]{\smash{{\SetFigFont{20}{24.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}1}%
}}}}
\put(1576,-286){\makebox(0,0)[lb]{\smash{{\SetFigFont{20}{24.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}2}%
}}}}
\put(2926,-736){\makebox(0,0)[lb]{\smash{{\SetFigFont{20}{24.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}3}%
}}}}
\put(2476,-2086){\makebox(0,0)[lb]{\smash{{\SetFigFont{20}{24.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}4}%
}}}}
\end{picture}%

